PDL on Steroids: on Expressive Extensions of PDL with Intersection and Converse

We introduce CPDL+, a family of expressive logics rooted in Propositional Dynamic Logic (PDL). In terms of expressive power, CPDL+ strictly contains PDL extended with intersection and converse (a.k.a. ICPDL) as well as Conjunctive Queries (CQ), Conjunctive Regular Path Queries (CRPQ), or some known extensions thereof (Regular Queries and CQPDL). We investigate the expressive power, characterization of bisimulation, satisfiability, and model checking for CPDL+. We argue that natural subclasses of CPDL+ can be defined in terms of the tree-width of the underlying graphs of the formulas. We show that the class of CPDL+ formulas of tree-width 2 is equivalent to ICPDL, and that it also coincides with CPDL+ formulas of tree-width 1. However, beyond tree-width 2, incrementing the tree-width strictly increases the expressive power. We characterize the expressive power for every class of fixed tree-width formulas in terms of a bisimulation game with pebbles. Based on this characterization, we show that CPDL+ has a tree-like model property. We prove that the satisfiability problem is decidable in 2ExpTime on fixed tree-width formulas, coinciding with the complexity of ICPDL. We also exhibit classes for which satisfiability is reduced to ExpTime. Finally, we establish that the model checking problem for fixed tree-width formulas is in \ptime, contrary to the full class CPDL+.

==> characterization_general.tex <==
%!TEX root = main.tex
\color{blue}
\section{Characterization}

{\bf
VERSION CON C DE VARIAS VARIABLES (PERO SOLO A NIVEL INICIAL, NO EN SUBFORMULAS). 
LO TENÍA CASI ESCRITO, ASI QUE LO DEJO ACÁ POR SI SIRVE PARA ALGO. SI NO, BORRARLO.
}

In this section we consider expressions of the form 
\begin{align*}
    C[x_1,\dots,x_n]
\end{align*}
where 
\AP
(1) $C$ is a finite set of ``""atoms""'' of the form $\pi'(x,x')$, where $\pi'$ is a {\CPDLp} "program" and $x,x' \in \Vars$; and
(2) for every, $1\leq i\leq n$, $x_i$ appears in some "atom" of $C$. Note that for $i\neq j$, $x_i$ may be equal or distinct from $x_j$. 

Notice we do not add $C[x_1,\dots,x_n]$ as a new rule of the grammar of \CPDL. Namely, all strict "subexpressions" of $C[x_1,\dots,x_n]$ are "formulas" and "programs" as described in section \ref{sec:prelim}.

As before, we define $\vars(C[x_1,\dots,x_nt]) \eqdef \bigcup_{\tau \in C} \vars(\tau)$.
Observe that $\set{x_1,\dots,x_n}\subseteq\vars(C[x_s,x_t])$.
%
The semantics $\dbracket{C[x_1,\dots,x_n]}_K$ of such "program" on a "Kripke structure" $K$ is the set of all tuples of "worlds" $(w_1,\dots,w_n) \in \worlds{K}$ such that for some mapping $f : \vars(\pi) \to \worlds{K}$ we have (1) $f(x_i) = w_i$ for all $1\leq i\leq n$, and (2) $(f(x),f(x')) \in \dbracket{\pi'}_K$ for each $\pi'(x,x')\in C$. Also as before, we often write $K,v_1,\dots,v_n\models C[x_1,\dots,x_n]$ for $(v_1,\dots,v_n)\in\dbracket{C[x_1,\dots,x_n]}_K$.

\begin{remark}\label{fewer-variables}
$K,v_1,\dots,v_k\models C[x,y,\dots,y]$ iff $K,v_1,v_2\models C[x,y]$, and $K,v_1,\dots,v_k\models C[x,x,\dots,x]$ iff $K,v_1\models C[x,x]$.
% and $v_2=v_i$ for all $2<i\leq n$.
\end{remark}

Let $\bar q=(q_1, \dotsc, q_k)$ be a tuple and let $1\leq i\leq k$. By $\bar q[i\mapsto r]$ we denote the tuple $(q_1, \dotsc, q_{i-1}, r, q_{i+1}, \dotsc, q_k)$.

\paragraph{$k$-ary simulation relation}
\AP
% Given two "Kripke structures" $K, K'$, and "worlds" $v_1, \dotsc, v_k$ and $v'_1, \dotsc, v'_k$ of $K$ and $K'$ respectively, we define the ""$k$-ary simulation relation"" (or ""$k$-simulation"") $(K,v_1, \dotsc, v_k) \intro*\pebblesim k (K',v'_1, \dotsc, v'_k)$
% $\phantomintro*\notpebblesim k$
%  if 
% \begin{enumerate}
%     \item\label{it:ksim:harmony} $\set{v_i \mapsto v'_i : 1 \leq i \leq k}$ is a homomorphism from $K|_{\set{v_1, \dotsc, v_k}}$ to $K'|_{\set{v'_1, \dotsc, v'_k}}$ \sidediego{definir} and 
%     \item\label{it:ksim:zig} for every $1 \leq i,j \leq k$\sidesanti{para que sirve pedir $i\neq j$?} with $i\neq j$, and every $\hat v_i$ in $K$ at "distance" $\leq 1$ from $v_j$, there must be some $\hat v'_i$ in $K'$ such that $(K,v_1, \dotsc, v_{i-1}, \hat v_i, v_{i+1}, \dotsc, v_k) \pebblesim k (K',v'_1, \dotsc, v'_{i-1}, \hat v'_i, v'_{i+1}, \dotsc, v'_k)$.
% \end{enumerate}
\AP
Given two "Kripke structures" $K, K'$, and tuples $\bar v=(v_1, \dotsc, v_k)\in \worlds{K}^k$ and $\bar v'=(v'_1, \dotsc, v'_k)\in \worlds{K'}^k$, we say that $K',\bar v'$ "$k$-simulates" $K,\bar v$, notated $K,\bar v \intro*\pebblesim k K',\bar v'$, if there is $H\subseteq \worlds{K}^k\times \worlds{K'}^k$ such that $\bar v H\bar v'$ and for all $\bar u=(u_1, \dotsc, u_k)\in \worlds{K}^k$ and $\bar u'=(u'_1, \dotsc, u'_k)\in \worlds{K'}^k$ such that $\bar uH\bar u'$:
\begin{enumerate}
    \item\label{it:ksim:harmony} $\set{u_i \mapsto u'_i : 1 \leq i \leq k}$ is a homomorphism from $K|_{\set{u_1, \dotsc, u_k}}$ to $K'|_{\set{u'_1, \dotsc, u'_k}}$ and 
    \item\label{it:ksim:zig} for every $1 \leq i,j \leq k$ with $i\neq j$, and every $\hat u_i$ in $K$ at "distance" $\leq 1$ from $u_j$, there is some $\hat u'_i$ in $K'$ such that $\bar u[i\mapsto \hat u_i] H \bar u'[i\mapsto \hat u'_i]$.
\end{enumerate}
Notice that by item \ref{it:ksim:harmony}, $\hat u'_i$ of item \ref{it:ksim:zig} is also at "distance" $\leq 1$ from $u_j'$.

For any $k' < k$, we will usually write $K,v_1, \dotsc, v_{k'} \pebblesim k K',v'_1, \dotsc, v'_{k'}$ to denote $K,v_1, \dotsc, v_{k'}, \underbrace{v_{k'}, \dotsc, v_{k'}}_{\text{$k-k'$ times}} \pebblesim k K',v'_1, \dotsc, v'_{k'},\underbrace{v'_{k'}, \dotsc, v'_{k'}}_{\text{$k-k'$ times}}$.


\begin{remark} \label{rk:pebblesim-shrink}
    If $K,v_1, \dotsc, v_k \pebblesim{k} K',v'_1, \dotsc, v'_k$ then $K,v_i, v_j \pebblesim{k} K,v'_i,v'_j$ and $K,v_i \pebblesim{k} K,v'_i$ for every $1 \leq i,j \leq k$. \sidediego{update to larger}
\end{remark}





\begin{theorem}\label{thm:charact-pos-sim}
    Let $k\geq 3$, let $K$ and $K'$ be "Kripke structures", let $\bar v=(v_1,\dots,v_k)\in \worlds{K}^k$ and let $\bar v'=(v'_1,\dots,v'_k)\in \worlds{K'}^k$. Consider the following two properties:
    \begin{enumerate}
        \item\label{thm:charact:pos} $K,\bar v\models C[x_1,\dots,x_k]\implies K',\bar v'\models C[x_1,\dots,x_k]$ for every positive %$\CPDLg{\+G_{\Tw[k-1]}}$-program 
        "program" $C[x_1,\dots,x_k]$ whose underlying graph has a "tree decomposition" of "tree-width" $\leq k-1$ with a bag equal to $\{x_1,\dots,x_k\}$; and

        \item\label{thm:charact:sim} $K,\bar v \pebblesim{k} K',\bar v'$.
    \end{enumerate}
    Then $\ref{thm:charact:sim}\implies\ref{thm:charact:pos}$, and if $K'$ is finitely branching then $\ref{thm:charact:pos}\implies \ref{thm:charact:sim}$.

% ENUNCIADO ORIGINAL
    % Let $k\geq 2$.
    % Given "Kripke structures" $K,K'$ and "worlds" $v,v'$ the following are equivalent
    % \begin{enumerate}
    %     \item for every "positive" $\CPDLg{\+G_{\Tw[k]}}$ formula $\phi$, we have $K,v \models \phi$ implies $K',v' \models \phi$; and
    %     \item $K,v \pebblesim{k+1} K',v'$;
    % \end{enumerate}
    % and the following are equivalent
    % \begin{enumerate}
    %     \item for every "positive" $\CPDLg{\+G_{\Tw[k]}}$ program $\pi$, we have $K,u,v \models \pi$ implies $K',u',v' \models \pi$; and
    %     \item $K,u,v \pebblesim{k+1} K',u',v'$.
    % \end{enumerate}
\end{theorem}


\begin{corollary}
    Let $k\geq 3$, let $K$ and $K'$ be "Kripke structures". Consider the following two properties:
    \begin{enumerate}
        \item\label{cor:charact:pos} $K,u,v\models \pi\implies K',u',v'\models \pi$ for every positive $\CPDLg{\+G_{\Tw[k-1]}}$-"program"; and

        \item\label{cor:charact:sim} $K,u,v \pebblesim{k} K',u',v'$.
    \end{enumerate}
    Then $\ref{cor:charact:sim}\implies\ref{cor:charact:pos}$, and if $K'$ is finitely branching then $\ref{cor:charact:pos}\implies \ref{cor:charact:sim}$.
    \end{corollary}
\begin{proof}
From Theorem \ref{thm:charact-pos-sim}, Remark \ref{fewer-variables} and the fact that $K,u,v\models C[x,y]\implies K',u',v'\models C[x,y]$ for every positive $\CPDLg{\+G_{\Tw[k-1]}}$-"program" $C[x,y]$ iff ($\{\pi[x,y]\}[x,y]\semequiv\pi$) $K,u,v\models \pi\implies K',u',v'\models \pi$ for every positive $\CPDLg{\+G_{\Tw[k-1]}}$-"program".
\end{proof}

\begin{corollary}
    Let $k\geq 3$, let $K$ and $K'$ be "Kripke structures". Consider the following two properties:
    \begin{enumerate}
        \item $K,u\models \phi\implies K',u',v'\models \phi$ for every positive $\CPDLg{\+G_{\Tw[k-1]}}$-formula; and

        \item$K,u \pebblesim{k} K',u'$.
    \end{enumerate}
    Then $\ref{cor:charact:sim}\implies\ref{cor:charact:pos}$, and if $K'$ is finitely branching then $\ref{cor:charact:pos}\implies \ref{cor:charact:sim}$.
    \end{corollary}


\begin{proof}[Proof of Theorem \ref{thm:charact-pos-sim}]
    We first show the 1-to-2 implication. 
   
    Assuming 1, we show that $K,\bar v\pebblesim{k}K,\bar v'$ via 
    \begin{align*}
    H&=\{(\bar u,\bar u')\mid K,\bar u\models C[\bar x]\implies K',\bar u'\models C[\bar x]\\
       & \mbox{ for any positive $\CPDLg{\+G_{\Tw[k-1]}}$-"program" $C[x_1,\dots,x_k]$}
    \\
        & \mbox{ whose underlying graph has a "tree decomposition"} 
    \\ & \mbox{of "tree-width" $\leq k-1$ with a bag equal to $\{x_1,\dots,x_k\}$}\}
    \end{align*}
    where $\bar u$ and $\bar u'$ are $k$-tuples of $\worlds{K}$ and $\worlds{K'}$ respectively and $\bar x=x_1,\dots x_k$. By 1, it is clear that $\bar vH\bar v'$.

    We next check that $H$ satisfies items \ref{it:ksim:harmony} and \ref{it:ksim:zig} of $\pebblesim{k}$. Item \ref{it:ksim:harmony} is straightforward. Let us see item \ref{it:ksim:zig}. Suppose by contradiction that there is $1 \leq i,j \leq k$ with $i\neq j$, and $v$ in $K$ at "distance" $\leq 1$ from $u_j$, such that for all $v'$ in $K'$ at "distance" $\leq 1$ from $u'_j$ we have $(\bar u[i\mapsto v],\bar u'[i\mapsto v'])\notin H$. Let $v'_1,\dots,v'_r$ be all the "worlds" in $K'$ which are at distance $\leq 1$ from $u'_j$ (there are finitely many because $K'$ is finitely branching). By the definition of $H$, for each $1\leq s\leq r$ there is a  
    positive $\CPDLg{\+G_{\Tw[k-1]}}$-"program" $\pi_s=C_s[\bar x[i\mapsto y_s]]$ such that
    $K,\bar u[i\mapsto v]\models \pi_s$,
    $K,\bar u'[i\mapsto v_s]\not\models \pi_s$, and
    the underlying graph of $\pi_s$ has a "tree decomposition" of "tree-width" $\leq k-1$ with a bag equal to $\{x_1,\dots,x_{i-1},y_s,x_{i+1},\dots,x_k\}$.
    Let $C$ be the set of all "atoms" in $C_s$ for any $1\leq s\leq r$ plus one of the following sets
    \begin{itemize}
    \item $\{x_j\to_ay_s\mid 1\leq s\leq r\}$ in case $u_j\to_av$ for $a\in\Prog$;

    \item $\{y_s\to_ax_j\mid 1\leq s\leq r\}$ in case $v\to_au_j$ for $a\in\Prog$;

    \item $\{\epsilon(x_j,y_s)\mid 1\leq s\leq r\}$ in case $u_j=v$.
    \end{itemize}
    and define $\pi=C[\bar x]$. One can check that that the "underlying graph" of $\pi$ has "tree-width" $\leq k-1$ and that 
    $K,\bar u\models \pi$ and
    $K,\bar u'\not\models \pi$, 
    contradicting the fact that $\bar uH\bar u'$.

-----------------------------------------------------
ESTO QUE SIGUE ES LA PRUEBA ORIGINAL (SEMI-REVISADA) CON EL ENUNCIADO DE CHARACT EN NEGRO

    \medskip

    We now show the 2-to-1 implication by structural induction on the expression.
    Assuming $K, \bar v \pebblesim {k+1} K', \bar v'$ via $H$ and $K,\bar v \models e$ for a "positive" $\CPDLg{\+G_{\Tw[k]}}$ expression $e$, we show $K',\bar v' \models e$.
    We assume the normal form of \Cref{lem:normal-form}.

    \proofcase{$e=p$ for $p\in\Prop$} If $K,v \models p$ then it follows that since there is a "homomorphism" mapping $v$ to $v'$ we have $K',v' \models p$.

    \proofcase{$e=a$ for $a\in\Prog$} If $K,u,v \models a$ then it follows that since there is a "homomorphism" mapping $u\mapsto u'$ and $v\mapsto v'$ we have $K',u',v' \models a$.

    \proofcase{$e=\bar a$ for $a\in\Prog$} Analogous as previous case.

    \proofcase{$e=\phi_1\land\phi_2$} If $K,v \models \phi_1\land\phi_2$ then for $i=1,2$ we have $K,v \models \phi_i$ and by inductive hypothesis we have $K',v' \models \phi_i$ for $i=1,2$, which implies $K',v' \models \phi_1\land\phi_2$.

    \proofcase{$e=\pi_1\cup\pi_2$} Similar as previous case. 

    \proofcase{$e=\phi?$} If $K,u,v \models \phi?$ then $u=v$ and $K,u \models \phi$. By inductive hypothesis $K',u' \models \phi$ and so $K',u',v' \models \phi$.

    \proofcase{$e=\tup{\pi}$} 
    If $K,v \models \tup{\pi}$ then there is some $\tilde v$ in $K$ such that $(v,\tilde v) \in \dbracket{\pi}_K$. Since (1) $v$ and $\tilde v$ are connected in $K$, (2) $(K, v) \pebblesim{k+1} (K', v')$ via $H$, and (3) $k+1 \geq 3$ it follows that there is some $\tilde v'$ such that  $(v,\tilde v) H (v', \tilde v')$. This can be obtained by ``navigating'' from $v$ to $\tilde v$ in $K$ using the definition of $\pebblesim{k+1}$.
    We can now apply the inductive hypothesis obtaining that $K',(v',\tilde v') \models \pi$, and thus that $K',v' \models \tup{\pi}$.

    \proofcase{$e = C[~]$} 
    We will actually work with the more general version of "programs" $C[\bar z]$ as introduced in \Cref{sec:to_ICPDL}.\sidesanti{not anymore...}
    Assume $\pi=C[x_1, \dotsc, x_t]$ with $t \leq k$, and suppose $\set{x_1, \dotsc, x_t}$ are pairwise distinct variables.
    %
    Let $(T,\bagmap)$ be a "tree decomposition" of $\uGraph{\pi}$ of "width" $k$, 
    with the assumption that
    for every pair of vertices $v_1,v_2$ in the same "bag", there is an edge from $v_1$ to $v_2$. 
    This is without loss of generality by Remark~\ref{rk:graph-programs-closed-minors}.
    
    Suppose $K,\bar v \models \pi$ and $K,\bar v \pebblesim{k+1} K',\bar v'$. 
    We will show $K',\bar v' \models \pi'$.
    Let $h$ be a "satisfying mapping" \sidesanti{definir} of $\pi$ on $K$. In particular, $\bar v = (h(x_1), \dotsc, h(x_t))$. We will show that there exists a "satisfying mapping" $h'$ of $\pi$ on $K'$.

    Suppose that the root $b$ of $T$ has $\ell$ children $b_1, \dotsc, b_\ell$, and let $T_1, \dotsc, T_\ell$ be the corresponding subtrees. Let $\bar y_i$ the vector of (pairwise distinct) variables containing $\bagmap(b_i) \cap \bagmap(b)$, that is, the variables which are both in the root "bag" of $T$ and in the "bag" of its $i$-th child. We can assume that $\bar y_i$ is of dimension $\leq k$ (otherwise parent and child would have exactly the same "bag").
    % in the same order as $(x_1, \dotsc, x_t)$. 
    Let $\bar v_i = h(\bar y_i)$.
    \santi{$h(\bar y_i)=(h({y_i}_1),\dots,h({y_i}_{|y_i|}))$ ?}
    Let $C_i \subseteq C$ be the set of all "atoms" contained in "bags" of $T_i$. Let $C_0$ the set of all "atoms" in the root bag, and let $\bar v_0 = \bar v$.
    \sidediego{an example is in order}
    It then follows that $K,\bar v \models C[x_1, \dotsc, x_t]$ if{f} $K,\bar v_i \models C_i[\bar y_i]$ for every $0 \leq i \leq \ell$.
    \begin{claim}
        Let $h(\bagmap(b)) = \set{h(x) : x \in \bagmap(b)}$.
        We have that there is a mapping $f : h(\bagmap(b)) \to \worlds{K'}$ such that
        (1) $K,\bar v_i \pebblesim{k+1} K',\bar v'_i$ for $\bar v'_i = f(\bar y_i)$ for every $i$, and (2) $\bar v' = (f(x_1), \dotsc, f(x_t))$. This is because of the "tree decomposition" assumption that every pair of elements of the root bag are at "distance" $\leq 1$,
        and of \Cref{rk:pebblesim-shrink}.
    \end{claim}
    We can now apply the inductive hypothesis since we have $K,\bar v_i \models C_i[\bar y_i]$ and $K,\bar v_i \pebblesim{k+1} K',\bar v'_i$, obtaining $K',\bar v'_i \models C_i[\bar y_i]$ for every $i$, which in turn means that $K',f(x_1), \dotsc, f(x_t) \models C[x_1, \dotsc, x_t]$.
    \santi{quizá a la $f$ convenga llamarla $h'$ o viceversa, por consistencia con lo que se dijo más arriba}

    \proofcase{$e = \pi^*$} If $\pi'=\pi^*$. Suppose $K, u,v \models \pi'$ and $K,u,v \pebblesim{k+1} K',u',v'$. We proceed by induction on the number of iterations. The base case $0$ corresponds to $K, u,v \models \pi^0$ which happens if and only if $u=v$, in which case $u'=v'$ by definition of $\pebblesim{k+1}$ and thus $K, u',v' \models \pi^0$.
    For the inductive case, $K, u,v \models \pi^n$. Note that $\pi^n$ is equivalent to $\tilde \pi = C[x_0,x_n]$ for $C = \set{\pi(x_i,x_{i+1}) : 0 \leq i < n}$. Since the subformulas of $\tilde \pi$ are the same as those of $\pi^*$ \sidesanti{esto es cierto?}(namely, $\pi$ and the subformulas therein), we can replace $\pi^n$ with $\tilde \pi$ and invoke the previous case, obtaining  $K',u',v' \models \pi^n$.

    \proofcase{$\pi \circ \pi'$} This case is similar to the case $\pi^*$.

\end{proof}



\paragraph{$k$-ary bisimulation relation}
\AP
The "$k$-bisimulation" notion $\intro*\pebblebisim k$ is obtained in a standard way, by requiring "$k$-simulation" in both senses. \sidesanti{esta frase la sacaria porque no es cierto para lógica modal, por ejemplo, y no estoy seguro de que valga acá tampoco.}


Given two "Kripke structures" $K, K'$, and tuples $\bar v=(v_1, \dotsc, v_k)\in \worlds{K}^k$ and $\bar v'=(v'_1, \dotsc, v'_k)\in \worlds{K'}^k$, we say that $K,\bar '$ is $k$-bisimilar to $K',\bar v'$, notated $K,\bar v \intro*\pebblebisim k K',\bar v'$, if there is $H\subseteq \worlds{K}^k\times \worlds{K'}^k$ such that $\bar v H\bar v'$ and for all $\bar u=(u_1, \dotsc, u_k)\in \worlds{K}^k$ and $\bar u'=(u'_1, \dotsc, u'_k)\in \worlds{K'}^k$ such that $\bar uH\bar u'$::
\begin{enumerate}
    \item[$1$.\ ]$\set{u_i \mapsto u'_i : 1 \leq i \leq k}$ is a homomorphism from $K|_{\set{u_1, \dotsc, u_k}}$ to $K'|_{\set{u'_1, \dotsc, u'_k}}$; 
    
    \item[$1'$.\ ] $\set{u_i \mapsto u'_i : 1 \leq i \leq k}$ is a homomorphism from $K'|_{\set{u'_1, \dotsc, u'_k}}$ to $K|_{\set{u_1, \dotsc, u_k}}$;

    \item[$2$.\ ]\label{it:kbisim:zig} for every $1 \leq i,j \leq k$ with $i\neq j$, and every $\hat u_i$ in $K$ at "distance" $\leq 1$ from $u_j$, there is some $\hat u'_i$ in $K'$ such that $\bar u[i\mapsto \hat u_i] H \bar u'[i\mapsto \hat u'_i]$; and

    \item[$2'$.\ ]\label{it:kbisim:zag} for every $1 \leq i,j \leq k$ with $i\neq j$, and every $\hat u'_i$ in $K'$ at "distance" $\leq 1$ from $u'_j$, there is some $\hat u_i$ in $K$ such that $\bar u[i\mapsto \hat u_i] H \bar u'[i\mapsto \hat u'_i]$.
\end{enumerate}


% Given two "Kripke structures" $K, K'$, and "worlds" $v_1, \dotsc, v_k$ and $v'_1, \dotsc, v'_k$ of $K$ and $K'$ respectively, we define the ""$k$-ary bisimulation relation"" (or ""$k$-bisimulation"") $(K,v_1, \dotsc, v_k) \intro*\pebblebisim k (K',v'_1, \dotsc, v'_k)$
% $\phantomintro*\notpebblebisim k$
%  if 
% \begin{enumerate}
%     \item[$1$.\ ] $\set{v_i \mapsto v'_i : 1 \leq i \leq k}$ is a homomorphism from $K|_{\set{v_1, \dotsc, v_k}}$ to $K'|_{\set{v'_1, \dotsc, v'_k}}$;
%     \item[$1'$.] $\set{v'_i \mapsto v_i : 1 \leq i \leq k}$ is a homomorphism from $K'|_{\set{v'_1, \dotsc, v'_k}}$ to $K|_{\set{v_1, \dotsc, v_k}}$;
%     \item[$2$.\ ] for every $1 \leq i,j \leq k$ with $i\neq j$, and every $\hat v_i$ in $K$ at "distance" $\leq 1$ from $v_j$, there must be some $\hat v'_i$ in $K'$ such that $(K,v_1, \dotsc, v_{i-1}, \hat v_i, v_{i+1}, \dotsc, v_k) \pebblebisim k (K',v'_1, \dotsc, v'_{i-1}, \hat v'_i, v'_{i+1}, \dotsc, v'_k)$; and
%     \item[$2'$.] for every $1 \leq i,j \leq k$ with $i\neq j$, and every $\hat v'_i$ in $K'$ at "distance" $\leq 1$ from $v'_j$, there must be some $\hat v_i$ in $K$ such that $(K,v_1, \dotsc, v_{i-1}, \hat v_i, v_{i+1}, \dotsc, v_k) \pebblebisim k (K',v'_1, \dotsc, v'_{i-1}, \hat v'_i, v'_{i+1}, \dotsc, v'_k)$.
% \end{enumerate}

\begin{theorem}\label{thm:characterization-bisim}
    Let $k\geq 2$.
    Given "Kripke structures" $K,K'$ and "worlds" $v,v'$ the following are equivalent
    \begin{enumerate}
        \item for every $\CPDLg{\Tw}$ formula $\phi$, $K,v \models \phi$ if{f} $K',v' \models \phi$; and
        \item $(K,v) \pebblebisim{k+1} (K',v')$;
    \end{enumerate}
    and the following are equivalent
    \begin{enumerate}
        \item for every $\CPDLg{\Tw}$ "program" $\pi$, $K,u,v \models \pi$ if{f} $K',u',v' \models \pi$; and
        \item $(K,u,v) \pebblebisim{k+1} (K',u',v')$.
    \end{enumerate}
\end{theorem}



\color{black}

==> cmd.tex <==
%!TEX root = main.tex
\newcommand{\longshort}[2]{#2}
\newcommand{\defn}[1]{\defstyle{#1}}
\newcommand{\pp}{\textup{PP}\xspace}
\newcommand{\pnplog}{\ensuremath{{\textup P}^{{\np}[\log]}\xspace}}
\newcommand{\shp}{\ensuremath{\#\textup{P}}\xspace}%
\newcommand{\pshp}{\ensuremath{\textup{P}^{\shp}}\xspace}%
% \newcommand{\pspace}{\textup{\sc PSpace}\xspace}
% \newcommand{\npspace}{{\sc NPSpace}\xspace}
% \newcommand{\expspace}{{\sc ExpSpace}\xspace}
% \newcommand{\np}{\textup{\sc NP}\xspace}
% \newcommand{\sharpp}{{\sc NP}\xspace}
% \newcommand{\conp}{{\sc coNP}\xspace}
% \newcommand{\ptime}{{\sc PTime}\xspace}
% \newcommand{\exptime}{{\sc ExpTime}\xspace}
% \newcommand{\nexptime}{{\sc NExpTime}\xspace}
% \newcommand{\logspace}{{\sc LogSpace}\xspace}
% \newcommand{\nlogspace}{{\sc NL}\xspace}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\complexity}[1]{\textup{\textsc{#1}}\xspace}
\newcommand{\compl}[1]{\textup{\textsc{#1}}}
\newcommand{\np}{\complexity{NP}}
\newcommand{\pspace}{\complexity{PSPACE}}
\newcommand{\npspace}{\complexity{NPSPACE}}
\newcommand{\exptime}{\complexity{EXP}}
\newcommand{\nexptime}{\complexity{NEXP}}
\newcommand{\nlog}{\complexity{NL}}

\definecolor{light-gray}{gray}{0.9}
\definecolor{light-yellow}{RGB}{255, 255, 220}
\newcommand{\proofcase}[1]{\noindent\colorbox{light-gray}{#1}~~}

\newcommand{\data}{\textit{data}}
\newcommand{\lbl}{\textit{lab}}

\newcommand{\dcup}{\mathop{\dot\cup}}
\newcommand{\+}[1]{\mathcal{#1}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
% \newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}


%% Abbreviations
\newcommand{\resp}[1]{[resp.~#1]}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\aka}{\textit{a.k.a.}\ }
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\cf}{\textit{cf.}}
\newcommand{\cum}{\textit{cum}\xspace}
\newcommand{\sth}{\text{ s.t. }}
\newcommand{\wrt}{\text{w.r.t.\ }}


\newcommand{\defstyle}[1]{\textbf{#1}}

% \newcommand{\dbracket}[1]{[\![ #1 ]\!]}

\newcommand{\eqdef}{\mathrel{\raisebox{-.05em}{\ensuremath{\stackrel{\textrm{\,def}}=}}}}


\newcommand{\FOtwo}{\textup{FO}^2}%

%%% LOGIC SDA macros %%%
\newcommand{\Until}{\mathbin{\textup{\textsf{U}}}}%
\newcommand{\Since}{\mathbin{\textup{\textsf{S}}}}%
\newcommand{\Next}{\textup{\textsf{X}}}%
\newcommand{\Future}{\textup{\textsf{F}}}%
\newcommand{\Going}{\textup{\textsf{G}}}%
\newcommand{\Eqdata}{\tup{\sim}}%
\newcommand{\NEqdata}{\tup{\not\sim}}%
% \newcommand{\Logic}{\ensuremath{\textup{ML}^\sim}\xspace}%
\newcommand{\SLogic}{\ensuremath{\textup{SDL}}\xspace}%
\newcommand{\pSLogic}{\ensuremath{\textup{pSDL}}\xspace}%
\newcommand{\Eqdatag}[1]{\mathop{\tup{\sim}_{\geq #1}}}%
\newcommand{\NEqdatag}[1]{\mathop{\tup{\not\sim}_{\geq #1}}}%
\newcommand{\Eqdatas}[1]{\mathop{\tup{{=}}_{#1}}}%
% \newcommand{\Eqdatas}[1]{\mathop{\mydiamond_{#1}}}%
% \newcommand{\clap}[1]{\makebox[0pt]{\hss#1\hss}}
% \newcommand{\mydiamond}{%
%   \sbox0{$\Diamond$}%
%   \usebox0\kern-.5\wd0\clap{\raisebox{.1ex}{\scalebox{.7}[1]{$=$}}}\kern.5\wd0%
% }
\newcommand{\NEqdatas}[1]{\mathop{\tup{\neq}_{#1}}}%
\newcommand{\Logicg}[1]{\ensuremath{\textup{ML}^\sim}_{#1}\xspace}%
\renewcommand{\phi}{\varphi}%
% \newcommand{\qd}{\text{qd}}
\newcommand{\subf}[1]{\textit{sub}(#1)}%

\newcommand{\OMIT}[1]{}

\newcommand{\Aut}{\mathcal{A}}


==> translation_proofs.tex <==
%!TEX root = main.tex


\begin{proof}[Proof of Theorem \ref{thm:translation_to_ICPDL}]
We first show
%
\begin{proposition}\label{prop:base_CQ}
If $\pi=D[\bar z]$ is a $\twtcpdl$-"program" ($|\bar z|\leq 3$) in simple normal form such that all "atoms" in $D$ are $\ICPDL$-formulas or $\ICPDL$-"programs", $T$ is a nice complete "tree decomposition" of $G_\pi$ with root $\{\bar z\}$ of width $\leq 2$ such that $\vars(T)=\vars(D)$, and $L=f(\pi,T_\pi)$ then 
%
\begin{enumerate}
\item for all $x\in\{\bar z\}$, $u\in\dbracket{D[x]}_K$ iff $u\in\dbracket{L(x)}_K$;
\item $(u,v)\in\dbracket{D[x,y]}_K$ iff $(u,v)\in\dbracket{L(x,y)}_K$ for $x,y\in\{\bar z\}$ and $x\neq y$.
\end{enumerate}
\end{proposition}

%\begin{enumerate}
%\item if $\bar z=x$ is a singleton then $G,u\modelsD[x]$ iff $G,u\models L(x)$;
%\item if $\bar z=(x_1,x_2)$ or $\bar z=(x_1,x_2,x_3)$ then 
%$G,u,v\models((x_i,x_j),D)$ iff $G,u,v\models L(x_i,x_j)$ for $i,j\in\{1,2,3\}$ and $i\neq j$.
%\end{enumerate}

\begin{proof}
We proceed by induction in $T$. 

Observe that if $e$ is an $\ICPDL$-"formula" or -"program" then $\tr(e)=e$.
 Suppose that $T$ is a single bag $R$. Then $L=L^R_0$ and:
\begin{itemize}
\item if $R=\{x\}$ then $D=\{\varphi(x)\}$ for some $\ICPDL$-"formula" $\varphi$ and $\pi[x]=\varphi(x)$. Since $\tr(\varphi)=\varphi$, $L_0^R(x)=L(x)=\varphi$ and we are done since $D[x]$ is logically equivalent to $\varphi(x)=L(x)$.

\item if $R=\{x<y\}$ then then we may assume wlog that $D=\{\varphi_x(x), \varphi_y(x), \tilde\pi(x,y)\}$ for some $\ICPDL$-"formulas" $\varphi_x,\varphi_y$ and some $\ICPDL$-"program" $\tilde\pi$ and $\pi[x]=\varphi_x(x)$, $\pi[y]=\varphi_y(y)$, and $\pi[x,y]=\tilde\pi(x,y)$. Observe that $\tr(\varphi_x)=\varphi_x$, $\tr(\varphi_y)=\varphi_y$ and $\tr(\tilde\pi)=\tilde\pi$.

Now $D[x,y]$ is logically equivalent to $\varphi_x(x)\land \varphi_y(y) \land \tilde\pi(x,y)$, which is logically equivalent to $\varphi_x?\circ \tilde\pi\circ\varphi_y?$, and this is logically equivalent to $L(x,y)$. 

Finally $D[x]$ is logically equivalent to $\varphi_x(x)\land \exists y.\varphi_y(y)\land\tilde\pi(x,y)$, which is logically equivalent to $\varphi_x\land \langle L(x,y)\rangle$ and this is logically equivalent to $L(x)$. The argument for $D[y]$ is analogous. 

\item if $R=\{x<y<z\}$ then we may assume wlog that 
\begin{align*}
D&=\{\varphi_x(x), \varphi_y(y), \varphi_z(z), \\
&\tilde\pi_{xy}(x,y), \tilde\pi_{yz}(y,z), \tilde\pi_{xz}(x,z)\}.
\end{align*}

On the one hand we reason as before and obtain that $D[x,y]$ is logically equivalent to 
\begin{align*}
&\tilde\pi_{xy}(x,y)\land\varphi_x(x)\land\varphi_y(y)\land\\
&\exists z.\bigwedge \{\varphi_z(z), \tilde\pi_{yz}(y,z), \tilde\pi_{xz}(x,z)\},
\end{align*}
which is logically equivalent to 
$$
\varphi_x?\circ  (\tilde\pi_{xy} \cap \tilde\pi_{xz}\circ\varphi_z?\circ \tilde\pi_{zy})\circ \varphi_y?,
$$
which is logically equivalent to $L(x,y)$. The reasoning for $D[x,z]$ and $D[y,z]$ is analogous.
On the other hand, $D[x]$ is logically equivalent to 
\begin{align*}
&\varphi_x(x)\land \exists y,z.\bigwedge \{\varphi_y(y), \varphi_z(z), \\
&\tilde\pi_{xy}(x,y), \tilde\pi_{yz}(y,z), \tilde\pi_{xz}(x,z)\}
\end{align*}
and this is logically equivalent to 
$\varphi_x\land \langle L(x,y) \rangle$ and also to $\varphi_x\land \langle L(x,z) \rangle$. Both are logically equivalent and both are logically equivalent to $L(x)$. The reasoning for $D[y]$ and $D[z]$ is analogous.
\end{itemize}

Suppose now that $T$ has root $R=\{\bar z\}$ and $R$ has children $B_1,\dots,B_n$ for $n>0$, for $B_i=\{z^{B_i}\}$. Let $T_i=T (B_i)$, 
$D^{B_i}=D | \vars(T_i)$, and
%
$L^{B_i}=f( D_i [\overline z^{B_i}] , T_i)$.
By inductive hypothesis, $L^{B_i}$ satisfies
% \begin{enumerate}
% \item for all $x\in\{\bar z^{B_i}\}$ $G,u\models(x,D^{B_i})$ iff $G,u\models L^{B_i}(x)$;
% \item $G,u,v\models((x,y),D^{B_i})$ iff $G,u,v\models L^{B_i}(x,y)$ for $x,y\in\{\bar z^{B_i}\}$ and $x\neq y$.
% \end{enumerate}
\begin{enumerate}
\item for all $x\in\{\bar z^{B_i}\}$, $u\in\dbracket{D^{B_i}[x]}_K$ iff $u\in\dbracket{L^{B_i}(x)}_K$;
\item $(u,v)\in\dbracket{D^{B_i}[x,y]}_K$ iff $(u,v)\in\dbracket{L^{B_i}(x,y)}_K$ for $x,y\in\{\bar z^{B_i}\}$ and $x\neq y$.
\end{enumerate}

Let $T'_i$ be the result of removing from $T$ the "subtrees@trees" $T_{i+1},\dots,T_n$. 
Let $D_i=D|\vars(T_i)$.
Observe that $T'_0=R$, $T'_n=T$, $D_0=D|\{\bar z\}$ and $D_n=D$
Using the same arguments as in the base case, it can be shown by induction in $n$ that $L^R_i(x)$, as defined by the algorithm, satisfies
%
% \begin{enumerate}
% \item for all $x\in\{\bar z\}$ $G,u\models(x,D_i)$ iff $G,u\models L^R_i(x)$;
% \item $G,u,v\models((x,y),D_i)$ iff $G,u,v\models L^R_i(x,y)$ for $x,y\in\{\bar z\}$ and $x\neq y$.
% \end{enumerate}
\begin{enumerate}
\item for all $x\in\{\bar z\}$, $u\in\dbracket{D_i[x]}_K$ iff $u\in\dbracket{L^R_i(x)}_K$;
\item $(u,v)\in\dbracket{D_i[x,y]}_K$ iff $(u,v)\in\dbracket{L^R_i(x,y)}_K$ for $x,y\in\{\bar z\}$ and $x\neq y$.
\end{enumerate}
and this concludes the proof.
\end{proof}
Then we show:
%
\begin{proposition}
For any expression $e$ of $\twtcpdl$: 
\begin{enumerate}
\item if $e=\varphi$ is a "formula" then $u\in\dbracket{\varphi}_K$ iff $u\in\dbracket{\tr(\varphi)}_K $;
\item if $e=\tilde\pi$ is a "program" $(u,v)\in\dbracket{\pi}_K$ iff $u\in\dbracket{\tr(\pi)}_K $.
\end{enumerate}
\end{proposition}
\begin{proof}
It follows by induction in $e$. 

% Observe that one of the base cases is when $e$ is a program of the form $C[\bar x]$ and 



% If $D[z_1,z_2]$ is a $\twtcpdl$-program ($|\bar z|=2$) such that  

% in simple normal form such that all atoms in $D$ are ICPDL-formulas or ICPDL-programs, 

% $T$ is a nice complete tree decomposition of $G_\pi$ with root $\{\bar z\}$ of width $\leq 2$ such that $\vars(T)=\vars(D)$, and $L=f(\pi,T_\pi)$ then 
% %
% \begin{enumerate}
% \item for all $x\in\{\bar z\}$, $u\in\dbracket{D[x]}_K$ iff $u\in\dbracket{L(x)}_K$;
% \item $(u,v)\in\dbracket{D[x,y]}_K$ iff $(u,v)\in\dbracket{L(x,y)}_K$ for $x,y\in\{\bar z\}$ and $x\neq y$.
% \end{enumerate}
% \end{proposition}




\end{proof}
\end{proof}
